Intuitive Surgical SurgToolLoc and SurgVU Challenges Results: 2022-2025

Robotic assisted (RA) surgery promises to transform surgical intervention. Intuitive Surgical is committed to fostering these changes and the machine learning models and algorithms that will enable them. With these goals in mind we have invited the surgical data science community to participate in a yearly competition hosted through the Medical Imaging Computing and Computer Assisted Interventions (MICCAI) conference. With varying changes from year to year, we have challenged the community to solve difficult machine learning problems in the context of advanced RA applications. Here we document the results of these challenges, focusing on surgical tool localization (SurgToolLoc) and surgical visual understanding (SurgVU). The publicly released dataset that accompanies these challenges is detailed in a separate paper arXiv:2501.09209 [1].

==> TeamDocs2022/BioMedIA/BioMedIA_orig.tex <==
%\documentclass{article}

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2020

% ready for submission
% \usepackage{neurips_2020}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2020}

% to compile a camera-ready version, add the [final] option, e.g.:
%    \usepackage[final]{neurips_2020}

% to avoid loading the natbib package, add option nonatbib:
    %  \usepackage[nonatbib]{neurips_2020}

%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinkshttps://www.overleaf.com/project/602bdb5e3638a47f00d58a2a
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{graphicx}
%\usepackage{amsmath}
%\usepackage{caption}
%\usepackage[font={small}]{caption}
%\usepackage{subcaption}
%\usepackage{wrapfig}
%\usepackage{enumitem}
%\usepackage{amsmath}
%\usepackage{tikz}
%\usetikzlibrary{shapes,arrows,positioning}
%\usetikzlibrary{mindmap}
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\captionsetup[table]{skip=10pt}
%\newcommand{\R}{\mathbb{R}}
%\bibliographystyle{unsrt}
% \title{Multi- Label Surgical Tool Classification in Endoscopic Videos}

% \author{% 
%    Aleksandr Matsun $\ast$ \\
%    Aleksandr.Matsun@mbzuai.ac.ae
%    \And
%    Mugariya Farooq $\ast$\\
%    Mugariya.Farooq@mbzuai.ac.ae
%     \And
%    Numan Saeed\\
%    Numan.Saeed@mbzuai.ac.ae
%    \And
%    Jose Renato Viera Restom \\
%    Jose.Viera@mbzuai.ac.ae
%     \And
%    Mohammad Yaqub\\
%    mohammad.yaqub@mbzuai.ac.ae\\~\\
%    \textbf{Mohamed bin Zayed University of Artificial Intelligence, Abu Dhabi, UAE}\\
%    Team BioMedIA-2022
% %   \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
% }
% %1- move fig 2 to appendix 
% %2- move some dice definitions to appendix 
% %3- connect best loss to medical image application 
% %4- re-phrase the discussion and conclusion section 
% %5- add insight to loss function with diff obj functions 

%\begin{document}
% \captionsetup[sufigure]{labelfont=small}

%\maketitle

\subsection{Bin Zayed University of Artificial Intelligence - Team BioMedIA}

Team Members: Aleksandr Matsun$\ast$, Mugariya Farooq$\ast$, Numan Saaed, Jose Renato Viera Restom and Mohammad Yaqub\\

%\noindent  Which categories did this team plan to submit to?\\ Surgical Tool Classification

%\noindent What was this team's general motivation and plan?

The team was focused on the task of tool classification but they targeted the localization task as well considering the extent to which the task of localization could help the classification problem. The authors experimented with the simple architectures like ResNet 50 first and planned to build on these simple architectures to increase the performance of the model. At the end, the team used a combination of two architectures: ConvNext and Yolov5 which helped them improve the performance metrics.

\subsubsection{Method Description}

The authors developed a method that localized different surgical instruments in surgical videos with a two-stage model, a detection foundation model based on YOLOv5 \cite{bochkovskiy2020yolov4} to derive the bounding boxes and a classifier based on the ConvNext \cite{liu2022convnet} architecture. 

%\noindent Summarize your method design and implementation in detail:\\
\begin{itemize}
    \item Architecture Design: The authors proposed a two-stage framework by combining two standard architectures YOLOv5 and ConvNext. Yolov5 was used for the task of object detection. ConvNext, on the other hand, was used for image classification. The training was organized in a way that would reduce the effect of noisy labels.
    
    \item Data Preprocessing: According to the authors, the dataset posed many challenges due to the following reasons:
    \begin{itemize}
        \item Dataset Imbalance: As per the data exploration done by the authors, the imbalance in the dataset was huge. The videos contained some instruments which appeared thousands of times as compared to the others which appeared only tens of times as shown in Figure~\ref{fig:dimb}. The authors balanced the dataset by sampling videos with different frame rates taking into account the types of tools present in each video. They also optimized (minimized) the standard deviation of the frequency of each tool in the resulting dataset.
        \item Presence of banners: The banners showed the tools used in the surgery, and as proposed by the authors, the removal of the banners was crucial as it could have caused the model to learn the labels from the banners and not actually identify the instruments for their proper classification.
        \item Noisy Labels: The authors, upon careful inspection of the videos in the dataset, discovered that some tools might never appear in the video even though the label suggested otherwise, which made the labels noisy and the training challenging.
    \end{itemize} 
\begin{figure}
 \centering
 \includegraphics[scale=0.23]{TeamDocs/BioMedIA/data_imb.png}
 \caption{Frequency of each tool across the whole dataset. The graph illustrates the frequent appearance of some tools compared to the other tools. This creates a huge imbalance in the dataset.}
  \label{fig:dimb}
\end{figure}
    
    \item Data Augmentation: Due to the nature of the dataset, where numerous frames were similar, the authors proposed different transformations that could help in training. Different types of augmentations were used for the detection model and the classifier model. For detection, the authors used mosaic augmentation, mixup augmentation, and random perspective transformations. On the other hand, for the classifier, the authors used random image flipping, rotation, and color jittering.
    \item Model Input(s): As an end-to-end model, the proposed framework was designed to have a video frame (RGB image) as an input. The frames were obtained by processing the video data provided.
    \item Model Output(s): For each of the input frames, the framework independently outputs a set of labels for surgical tools present in the respective frame.
    \item Model Loss Function: The authors used a combination of box regression loss and objectness loss in order to train the localization model and a focal loss as the criterion for the classifier in order to partially mitigate the impact of the huge class imbalance in the dataset.
    \item Model Pretraining: The authors maintained that pretraining the model on different datasets that had similar characteristics as the provided data would, to some extent, boost the performance of the models. They trained ResNet50 and ConvNext on Cholec 80 \cite{twinanda2016endonet} and M2CAI \cite{jin2018tool}. Cholec 80 dataset consists of 80 cholecystectomy surgeries. The labels present are primarily phase and tool presence annotations, where the ground truth for phase annotations is shown in Figure \ref{fig:cholec} and has been confirmed by a surgeon. On the other hand, the m2cai16-tool-locations dataset contains 15 videos with tool annotations for seven surgical instruments, as shown in Figure \ref{fig:m2cai}. The labels are given per frame for 7 classes for each video.

\begin{figure}
 \centering
 \includegraphics[scale=0.35]{TeamDocs/BioMedIA/cholec.jpeg}
 \caption{Surgical instruments present in Cholec80 Dataset. The tools are similar to the tools present in the challenge dataset. }
  \label{fig:cholec}
\end{figure}


\begin{figure}
 \centering
 \includegraphics[scale=0.32]{TeamDocs/BioMedIA/m2kai.jpeg}
 \caption{Surgical instruments present in M2CAI Dataset. Some of the tools present are similar to the ones present in the given dataset.  }
  \label{fig:m2cai}
\end{figure}

\end{itemize}\\
%\noindent Describe how your method works for tool presence classification.\\
For the task of classification, out of various CNN architectures, ConvNext-Small provided the best results. However, the authors made the following assumptions about the data:
\begin{enumerate}
    \item They considered and filtered frames where all three instruments were present. They assumed that these frames were sufficient for the task of classification. They also assume that the distribution of surgical tools in these frames would be approximately the same as that in the actual dataset.
    
    \item In the vast majority of frames, the order in which the tools are listed on the label of a clip corresponds to the counter-clockwise order of their positions, starting from the upper left corner and ending with the upper right corner.
\end{enumerate}
Training algorithm: The authors used the localization model Yolov5 pretrained on a combination of three datasets:  EndoVis'15 Instrument Subchallenge Dataset, CholecSeg8k \cite{hong2020cholecseg8k} and Endoscopic instrument segmentation with crowdsourced data challenge dataset \cite{maier2014can} to detect the surgical tools in a frame with bounding boxes. The bounding boxes were saved as separate images alongside their respective image-level ID number derived from their position relative to the center of the image in an anti-clockwise fashion. The bounding boxes are then assigned the labels from the corresponding video clip (from left to right, depending on the id number of the bounding box). The outputs obtained were a set of predictions for the tools in the frame.
\noindent (optional) Figure of the model architecture\\
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{TeamDocs/BioMedIA/yoloplusclass.png}
    \caption{Architecture of the two-tier model used for classification. Images are passed through Yolov5 for generating bounding boxes around the tools. Then they are passed to ConvNext for classification.}
    \label{fig:archi}
\end{figure}

\subsubsection{Model Training}
%\noindent Training hyper-parameters:\\
To train the detection model, the authors used a batch size of 128, a learning rate of 0.001, and a total number of epochs 300. The classifier was using a batch size of 128, a learning rate of 0.0001 and the number of epochs was set to 5 due to fast convergence of the network.

%\noindent Hardware settings for compute, CPU, GPU:\\
Given the size of the dataset, the authors used a cluster to run their experiments on a GPU with 2x AMD EPYC 7742 CPUs (128 cores total with 256 threads), 256GB RAM, 4x Nvidia A100 SXM 40G GPUs.

\subsubsection{Preliminary Performance}

%\noindent Training, Validation and Testing Performance:\\
The performance of the model during training was quite high with models like ResNet-50 and ConvNext. When pretrained on the Cholec-80 dataset, ResNet produced a training F1 score of 0.989, while for ConvNext it was 0.985. Moreover, both of them produced around the same F1 scores when trained on M2CAI dataset. The authors believe that the unrealistically high-performance metrics were due to the similarity across the frames in different surgeries and the usage of the same set of tools for different surgeries with the same background. The validation performance for ConvNext-Small and the proposed two-tier model is shown in Table~\ref{table:loss_exps}. However, the testing performance for the proposed architecture was around 0.552.

\begin{table}[h]

\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
Model & F1-Score & Accuracy \\
\midrule
ResNet-50 & $0.20$ & $0.10$ \\
ConvNext-S  & $\textbf{0.83}$ & $0.39$ \\
Yolov5+ConvNext-S & $0.75$ & $\textbf{0.50}$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{Comparison of different models on the performance metrics. Models were pretrained on Cholec 80 and M2CAI.}
\label{table:loss_exps}
\end{table}


%\clearpage


%\bibliography{references}


 

%\small

% [1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
% connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
% (eds.), {\it Advances in Neural Information Processing Systems 7},
% pp.\ 609--616. Cambridge, MA: MIT Press.

% [2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
%   Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
% TELOS/Springer--Verlag.

% [3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
% recall at excitatory recurrent synapses and cholinergic modulation in rat
% hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.

%\end{document}

==> TeamDocs2022/HKMV/HKMV_original.tex <==

%
\subsection{South China University of China - Team HKMV}
% first person, past tense

\noindent Team Member: Weiliang Chen

\subsubsection{Method Description}

In order to obtain an object detection model that can effectively locate surgical tools, the key point is how to build a well labeled training dataset at a low cost. We used two public datasets endovis17 \cite{hkmv01} and endovis18 \cite{hkmv02} to assist us obtain a primary training dataset. We convert the clevis part in the mask label of the dataset into a bounding box label, and train an object detection model. We use this model to infer the images of the competition dataset and then adjust the predicted bounding box slightly. After repeating several operations, we can obtain a large-scale training dataset. 

In terms of model, we build a two-stage object detection model based on faster-rcnn. We choose efficientnet-b3, which takes into account both performance and speed, as the backbone to extract image features, and add FPN structure to further optimize the feature map.\\

\noindent{Dataset:}

We used two public dataset endovis17 and endovis18 to assist us obtain a primary training dataset. These two data sets provide mask annotations, as shown in the following figure \ref{data}.

\begin{figure}[tbh]
\caption{data description figure}\label{data}
\centering
\includegraphics[width=0.7\textwidth]{TeamDocs/HKMV/hkmv01Fig.pdf}
\end{figure}

We convert the clevis part in the mask label of the dataset into a bounding box label and use them as the primary training dataset. Since endovis17 and endovis18 does not include all 14 surgical tools, we have added a small part of data to the training dataset to ensure that the dataset contains all 14 surgical tools. Finally, our dataset contains 5212 images.\\

\noindent{Surgical Tool Localization Algorithm:}
\begin{itemize}
\item a) We train a faster-rcnn object detection model on the primary training dataset.
\item b) We choose efficientnet-b3, which takes into account both performance and speed, as the backbone to extract image features, and add FPN structure to further optimize the feature map.
\item c) According to the size of the clevis of surgical tools in the training dataset, we designed four layers of feature maps for the model, which downsampling 8, 16, 32 and 64 times respectively.
\end{itemize}

\noindent{Dataset Expansion and Adjustment:}

\begin{figure}[tbh]
\caption{model architecture}
\centering
\includegraphics[width=0.7\textwidth]{TeamDocs/HKMV/hkmv02Fig.pdf}
\end{figure}

In order to increase the size of the dataset, we use the trained model to infer the images of the competition dataset, and add the inferential images to the training dataset. We use a score threshold of 0.7 to filter out the poor bounding box and then adjust the predicted bounding box slightly, which is a very low labor cost operation. After several expansion operations, we expanded the dataset to 11035 images. The dataset expansion flow diagram of our algorithm is as follows:

\begin{figure}[tbh]
\caption{data expansion scheme}
\centering
\includegraphics[width=0.7\textwidth]{TeamDocs/HKMV/hkmv03Fig.pdf}
\end{figure}

%\subsubsection{Model Training}

\subsubsection{Preliminary Performance}

We extracted 25\% from the dataset as the validation dataset, and ensured that the data of validation dataset were all from the original well labeled images, so as to correctly evaluate our algorithm. We tested many model parameters, and finally chose the model structure of efficientnet-b3 as the backbone, downsampling 8, 16, 32, 64 times of the feature map. On our validation dataset, our model can reach a mean mAP of 0.452.

==> TeamDocs2022/HRI_MV/HRI_MV_original.tex <==

\subsection{Hikvision Research Institute - Team HRI\_MV}
% first person, present tense
\noindent Team Member: Quan He\\

The data set provided by the competition does not contain detection box labels, so we need to use weak supervision or semi supervision to train our model. We make full use of the characteristics of the video data and adopt a object tracking scheme with a Semantic segmentation network to obtain the pseudo tags of the frames. In particular, we use the IOU scoring mechanism with the dual model cross validation mechanism to choose more reliable pseudo tags. Using the obtained pseudo tags, we train the detector, integrate the tracker and detector into a pseudo tag using Kalman filter, and iteratively update the models.

In traditional instrument target detection, the whole of the object is considered as GT and included in the detection frame, while in surgical instrument detection, only clevis is considered as GT. The difficulty is that the appearance of clevis of different devices is relatively similar. When human eyes distinguish different devices, they are actually mainly distinguished according to the clamps of the devices. To solve this problem, we modify the ROI proposal box output by RPN network. For the regression head, we use the proposal box output by RPN, while for the classification head, we expand the proposal box to obtain more information for device classification.

Finally, we use the integration algorithm to use the detection frame output from the previous frame for target tracking, and integrate the results of target detection and target tracking by weighting, which effectively solves the problem of target missing detection.

\subsubsection{Method Description}

\noindent{Object Tracking with Cross Supervision:}

We choose to label the picture sequence of the video by using the method of target tracking. We manually label the first frame of the video and automatically label the subsequent frames using the target tracking algorithm. However, the tracking process sometimes fails. We found that this was caused by clevis’ small and inconspicuous features, reflection and other factors. Therefore, we propose a cross validation method based on segmentation results. 

Specially, We chose siamfc\texttt{++}[1] For single target tracking (SOT), the advantage of this scheme is that we can directly use the trained sot model without retraining. We only need to label the first frame of the picture sequence, and sot can track the subsequent picture frames effectively.Then, we train a unet-like segmentation network with the open source data dVRK segmentation dataset [2],Event-based-2D-tracking-of-articulated-instruments-for-robotic-surgery dataset[3],EndoVis17 dataset [4], EndoVis18 dataset [5]

We calculate the IOU between the tracking box and the segmentation result. For frames with IOU less than the threshold value of 0.2, we think that the tracking fails or the generated pseudo label is untrustworthy. We remove this part of false tags and track the previous boxes. If the box keeps crashing, we will mark it manually again.

We train the detector with a part of pseudo labels, and then use the detector to generate pseudo labels with the above tracking output to get new labels. In this way, we finally obtain a dataset containing about 25000 pictures with pseudo labels.

\noindent{Roi Expand:}

We choose cascade RCNN [6].As a target detection model. In the initial test results, we found that although many instruments were successfully detected, they were misclassified. This is because in traditional instrument target detection, the whole of the object is considered as GT and included in the detection frame, while in surgical instrument detection, only clevis is considered as GT, and the appearance of clevis components of different instruments is relatively similar, and the difference is mainly reflected in the clamp part.

To solve this problem, we modify the ROI proposal box output by RPN network. For the regression head, we use the proposal box output by RPN, while for the classification head, we expand the proposal box twice in width and height, respectively, to obtain more information for device classification, as shown in the following figure.

\begin{figure}[tbh]
\caption{The information required for detection and classification is different}\label{fig1}
\centering
\includegraphics[width=0.2\textwidth]{TeamDocs/HRI_MV/HRI_MV_Fig1.pdf}
\end{figure}

In order to verify that our ideas are correctly understood by the model, the following figure2 shows the feature map extracted from the backbone of our model. In the original model, the instrument cadiere forceps was mistakenly considered prograsp Forceps and tip up fenestrated Grasper, the thermodynamic values in its characteristic diagram are all concentrated in clevis. And in our proposed ROI In the expand model, cadiere forceps is correctly classified, and in its feature map, there is not only a large thermal value distribution at the clevis, but also a large thermal value at the clamp, which helps our model to better classify instruments.

\begin{figure}[tbh]
\caption{ROI expand makes model identification device}
\centering
\includegraphics[width=0.6\textwidth]{TeamDocs/HRI_MV/HRI_MV_Fig2.pdf}
\end{figure}

\noindent{Model ensemble:}

In addition, we find that sometimes the model may miss detection. In order to solve this problem, we use the detection frame output from the previous frame algorithm for target tracking, and integrate the results of target detection and target tracking by weighting. In this way, as long as the device appears in a certain frame, it can be identified by target tracking in its subsequent picture frames, effectively solving the problem of target missing detection.
The overall framework of our algorithm is shown in the figure 3 below

\begin{figure}[tbh]
\caption{model ensemble}
\centering
\includegraphics[width=0.4\textwidth]{TeamDocs/HRI_MV/HRI_MV_Fig3.pdf}
\end{figure}

\subsubsection{Preliminary Performance}\\
We first established a test set to verify the performance of the detector to evaluate whether we need more data. The test set is determined by manual review to include each sample category. Roundn means the n times we use Object tracking with Cross Supervision method to get more data (see table below). %\ref{table:hri_mv1}).

\begin{table}[tbh]
\begin{center}
\begin{tabular}{lllll}
\hline
Method & Round1 & Round2 & Round3 & Round4  \\ \hline
mean mAP & 0.164 & 0.347 & 0.489 & 0.491 \\ \hline
\end{tabular}
%\caption{Table}
%\label{table:hri_mv1}
\end{center}
\end{table}

By the fourth round, our performance has improved slightly. We use this data for the next experiment. We divide all the data into training set and test set (7:3) to verify what strategies we can take to enhance the performance of the model (table \ref{table:hri_mv}).

\begin{table}[tbh]
\begin{tabular}{ll}
\hline
Method                      & mean mAP  \\ \hline
Base              & +0.489      \\
+ swin pretrained \cite{hri_mv7} & +0.052      \\
+ roi expand 2            & +0.063      \\
+ ChannelShuffle-RGNShift  & +0.021      \\
+Fog-Blur-Noise         & +0.048      \\
+ focallosss           & +0.002      \\
+cbam\cite{hri_mv8}              & +0.033      \\
+DetecoRS pretrained \cite{hri_mv9} & +0.059      \\
swin pretrained + roi expand 2 + Fog-Blur-Noise + ChannelShuffle-RGBShift &    +0.109      \\
detectors pretrained + roi expand 2 + Fog-Blur-Noise + ChannelShuffle-RGBShift               & +0.111      \\ \hline
\end{tabular}
\caption{Model Results}
\label{table:hri_mv}
\end{table}

We prove that some strategies can improve the performance of the model on the current test set, while some cannot. And  by adopting ROI expand method,the the overall performance improved by 0.063.

We finally selected the last two models in the table as the models for ensemble. On the Surgical tool localization Leaderboard，We have confirmed the effectiveness of the ensemble scheme. The single model reached a score of 0.3985 on the final test set, while the ensemble model reached a score of 0.4077 and ranked the first. Since the detector can classify the target ,we also join in the Surgical tool detection Tasks.However, on the Surgical tool detection Leaderboard, The performance of ensemble model is not as good as that of single model, the former score is 0.7485 and the latter is 0.7341.



==> TeamDocs2022/HVRL/HVRL_orig.tex <==
% This is samplepaper.tex, a sample chapter demonstrating the
% LLNCS macro package for Springer Computer Science proceedings;
% Version 2.20 of 2017/10/04
%
%\documentclass[runningheads]{llncs}
%
%\usepackage{graphicx}
%\usepackage{graphicx}
%\usepackage{comment}
%\usepackage{color}
%\usepackage{multirow}
%\usepackage{makecell}
%\usepackage{cite}
%\usepackage{bm}
%\usepackage{amsmath,amssymb}
%\newcommand{\etal}{\textit{et al}. }
%\usepackage{url}
% Used for displaying a sample figure. If possible, figure files should
% be included in EPS format.
%
% If you use the hyperref package, please uncomment the following line
% to display URLs in blue roman font according to Springer's eBook style:
% \renewcommand\UrlFont{\color{blue}\rmfamily}

%\begin{document}
%
%\title{Surgical Tool Localization in endoscopic videos}


%\author{Ryo Fujii \and
%Ryo Hachiuma \and
%Mana Masuda \and
%Hideo Saito
%}
%\authorrunning{R. Fujii et al.}

%\institute{Keio University, Yokohama, Kanagawa, Japan \\
%\{ryo.fujii0112, ryo-hachiuma, mana.smile, hs\}@keio.jp }


\subsection{Team HVRL}

\noindent who are the members of this team? \\
Ryo Fujii, Ryo Hachiuma, Mana Masuda and Hideo Saito

\noindent which categories did this team plan to submit to? \\
Both category1 and 2

\noindent what was this team's general motivation and plan? \\
The main motivation is to familiarize ourselves with weakly supervised learning in a real surgery environment. We have an experience to build the large scale tool presence detection dataset in open surgery and deeply understand how expensive and tedious to   annotate the surgery video \cite{app122010473}. Thus, we are interested in applying the weakly supervised learning which reduce the annotation time to a real surgery video.


\subsubsection{Method Description}
\noindent concise overview of the proposed method, include motivation and novelty. \\
\noindent summarize your method design and implementation in details:\\

For category1, we trained the multi-label tool presence classification models in a fully supervised manner. Since only video clip-wise annotation is provided, we assume all frames in a video clip has the same annotation as the annotation attached to the video clip. Our solution is the ensemble of three different models, Swin Transformer V2 \cite{Liu_2022_CVPR}, EfficientNetV2 \cite{pmlr-v139-tan21a}, and ResNeXt \cite{DBLP:journals/corr/XieGDTH16} , which showed the high performance to the validation data. We implemented the models based on the PyTorch Image Models \url{https://github.com/rwightman/pytorch-image-models} \cite{rw2019timm}. 

For category2, We employ Grad-CAM++~\cite{8354201} for the weakly-supervised tool localization task.

\begin{itemize}
    \item architecture design
    
    For category1, we adopt the ensemble of three different models, Swin Transformer V2 \cite{Liu_2022_CVPR}, EfficientNetV2 \cite{pmlr-v139-tan21a}, and ResNeXt \cite{DBLP:journals/corr/XieGDTH16}.

    For category2, We only employ EfficientNetV2.
    \begin{figure*}[tb]
\begin{center}
\begin{tabular}{ccc}
\begin{minipage}{0.3\hsize}
    \begin{center}
        \includegraphics[trim={0 1em 0 0}, clip, width=\hsize]{TeamDocs/HVRL/original.jpg} 
    \end{center}
\end{minipage}
&
\begin{minipage}{0.3\hsize}
    \begin{center}
        \includegraphics[trim={0 1em 0 0}, clip, width=\hsize]{TeamDocs/HVRL/crop.jpg} 
    \end{center}
\end{minipage}
&
\begin{minipage}{0.3\hsize}
    \begin{center}
        \includegraphics[trim={0 1em 0 0}, clip, width=\hsize]{TeamDocs/HVRL/blur.jpg}
    \end{center}
\end{minipage}
\\
{\footnotesize (a) Original image}
&
{\footnotesize (b) UI cropped image}
&
 {\footnotesize (c) UI blurred image}
\end{tabular}
\caption{Examples of preprocessing. The original image includes the black region on the left and right sides and the tool annotation UI on the bottom. Firstly, we crop the original image to remove the black region. Then, we randomly conduct either of two procedures, UI cropping or UI blurring with a probability of 0.5.}
\label{fig:1}
\end{center}
\end{figure*}
    \item data processing, reformatting, transformation, etc. (if any)  \\
    The image extracted from video clips includes a black region on the left and right sides and a tool annotation UI on the bottom. Firstly, we remove these black regions. Then,
we randomly conduct either of two procedures, UI cropping or UI blurring with a
probability of 0.5. These procedures prevent the model from getting the tool presence information from the UI directory. Examples are shown in Fig. \ref{fig:1}.



    \item data augmentation (if any) 
    
    We apply several data augmentation techniques for achieving robust training. Specifically, we apply the data augmentation shown in Table \ref{tab:aug}.  These augmentations are applied to train all models.
    \item model input(s)  
    
    RGB image.
    \item model output(s)  
    
    For category1, multilabel output.
    For category2, pixel-wise heatmap.
    \item model loss function  
    
    For category1, binary cross-entropy loss.
    
    For category2, we utilize the model trained by category1., so we do not conduct a training.
    \item temporal components (if any) 
    
    Nothing.
    \item model pre-training (if used) 
    
    For category1, The weights of Swin Transformer V2 and EfficientNetV2 are initialized with the weights trained with ImageNet \cite{deng2009imagenet}, and that of ResNeXt is initialized with the weights trained with Instagram Datasets.

    For category2, we utilize the model trained by category1., so we do not conduct a training.
    \item transfer learning technique (if used) 
    
    Nothing.
    \item post-propcesing (if any) 
    
    For category1, at the test-time, we employ test-time augmentation scheme. We flip the test image. As a result, we augment the single image to twop images and merge the prediction against two images.

    For category2, we compute the gradient for the last convolutional layer and penultimate convolutional layer via the back-propagation. After obtaining the pixel-wise heatmap for each layer, we average these two heatmaps to obtain the final heatmap. Then, we binarize the heatmap with threshold $\sigma=0.5$ to obtain the binary map. Finally, we apply connected component algorithm to extract multiple bounding boxes from the binarized heatmap.
\end{itemize}
\noindent describe your method works for tool presence classification.\\
The trained model output a multi-class label. \\ 
\noindent describe how your method works for tool localization.\\
The Grad-CAM++~\cite{8354201} module generate the class activation maps. Then, we binarize the the the generated class activation maps with threshold $\sigma=0.5$ to obtain the binary map. Finally, we apply connected component algorithm to extract multiple bounding boxes from the binarized heatmap.

\noindent (optional) figure of the model architecture\\
\noindent (optional) pseudo algorithm table \\

\subsubsection{Model Training}

\subsubsection{Preliminary Performance}
\begin{table}[tb]
\centering
\caption{Local validation results with different models.}
\begin{tabular}{c|c}
\hline \Xhline{2\arrayrulewidth}
Method & F1-score \\ \hline
Swin Transformer V2 &  0.925 \\
EfficientNetV2  & \textbf{0.930}\\ 
ResNeXt & 0.928 \\
Model ensemble & \textbf{0.930} \\
\hline \Xhline{2\arrayrulewidth}
\end{tabular}
\label{tab:res}
\end{table}
\noindent training, validation, testing performance\\
We summarize the results against the local validation data at Table \ref{tab:res}. We choose the models which showed the best performance on our local validation data. Specifically, the number of epochs is 17, 25, and 23 respectively. We can observe that a single EfficientNetV2  and the ensemble of three models show the highest score on the F1 score. 

\noindent (optional) table of performance results \\
Shown in Table \ref{tab:res}. 


\begin{table}[tb]
\centering
\caption{Hyperparameters}
\begin{tabular}{cccc}
\hline \Xhline{2\arrayrulewidth}
methods & learnign rate & batch size & epochs \\ \hline
Swin Transformer V2  & 0.6  & 24 & 50 \\
EfficientNetV2 & 0.57 & 48 & 30 \\
ResNeXt  & 0.36 & 192 & 50 \\
\hline \Xhline{2\arrayrulewidth}
\end{tabular}
\label{tab:1}
\end{table}

\noindent training hyer-parameters, batch size, total epoch/iteration, random seed (if any).\\
For category1, we employ Stochastic Gradient Descent Optimize with the momentum $0.9$, weight decay $0.0001$, 
 and 
cosine annealing strategy. For the learning rate, batch size, and training epochs, we use different settings on three methods as shown in Table \ref{tab:1}.  

For category2, we utilize the model trained by category1., so we do not conduct a training.

\noindent data preparation, pre-processing, etc.\\
As mentioned above, as pre-processing, we crop the
original image to remove the black region. Then, we randomly conduct either of two
procedures, UI cropping or UI blurring with a probability of 0.5.


\noindent hardware settings for compute, CPU, GPU, etc. \\
NVIDIA RTX A5000 






\begin{table}[tb]
\centering
\caption{Data augmentation}
\begin{tabular}{ccc}
\hline \Xhline{2\arrayrulewidth}
Augmentation & Range & Probability \\ \hline
Horizontal flip & & 0.5\\
Color shift & 30 & 0.5\\
HSV Shift & 20 & 0.5\\
Brightness &[0.1, 0.3] & 0.2\\
\hline \Xhline{2\arrayrulewidth}
\end{tabular}
\label{tab:aug}
\end{table}


%\bibliographystyle{splncs04}

%\bibliography{ref}
%\end{document}


==> TeamDocs2022/NVIDIA/NVIDIAold.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\usepackage{graphicx}

%\title{SurgToolLoc 2022 Team NVIDIA}
% \author{ }
%\date{January 2023}

%\begin{document}

%\maketitle


%\section{Section Name}

% we are asked to fill out the subsection below

\subsection{Team NVIDIA}

\noindent who are the members of this team?\\

Bo Liu, David Austin, Yiheng Wang, Michal Futrega, Jean-Francois Puget \\

\noindent which categories did this team plan to submit to?\\

Both categories. \\

\noindent what was this team's general motivation and plan?\\

This team consists of five NVIDIA employees. Three of them (Jean-Francois, David and Bo) are members of the Kaggle Grandmasters team, with extensive experience in computer vision machine learning competitions. One member (Yiheng) works on MONAI, NVIDIA's medical imaging toolkit. Another (Michal) works on building GPU optimized models for NVIDIA's Deep Learning Examples repository\footnote{https://github.com/NVIDIA/DeepLearningExamples}. This team's motivation was to win prize in both categories using NVIDIA software stack. \\

\subsubsection{Method Description}
% \noindent concise overview of the proposed method, include motivation and novelty. \\
% \noindent summarize your method design and implementation in details:\\
% \begin{itemize}
%     \item architecture design
%     \item data processing, reformatting, transformation, etc. (if any)
%     \item data augmentation (if any)
%     \item model input(s)
%     \item model output(s)
%     \item model loss function
%     \item temporal components (if any)
%     \item model pre-training (if used)
%     \item transfer learning technique (if used)
%     \item post-propcesing (if any)
% \end{itemize}
% \noindent describe how your method works for tool presence classification.\\
% \noindent describe how your method works for tool localization.\\
% \noindent (optional) figure of the model architecture\\
% \noindent (optional) pseudo algorithm table \\

Task 1 is a weakly supervised task in the sense that classification labels are given on video level instead of frame level, but test predictions need to be performed on frame level. Since many video level tools don’t appear in all the frames of the video, the major challenge of task 1 is to identify frames which contain clean labels. They came up with a unique way to tackle this: first use segmentation models to identify frames where they could identify three unique tools per frame. By identifying three tools, they could then apply the video level labels to the given frame. In order to do this they used models \cite{shvets2018automatic} published from the MICCAI 2017 Robotic Instrument Segmentation Challenge\footnote{https://github.com/ternaus/robot-surgery-segmentation}. After applying
segmentation models they then used traditional computer vision techniques to count the contours of each unique instrument, and layered additional logic (i.e., instrument contour needs to touch
frame edge) to filter out false positives. All frames where they could positively identify three unique instruments per frame then formed the basis of the training dataset. \\

Another unique thing in this dataset is the fact that many videos are sequential, e.g., 30 second chunks of a continuous video that last for several minutes or even dozens of minutes. Grouping
videos from the same “scene” into the same fold split is critical for meaningful local validation. In order to do this, they compared the image hash of each video’s first frame and the last frame of the preceding video. If the similarity is lower than a threshold, they mark them as from the same scene, and put all videos of the same scene into the same split when they split the data into 5 folds. This way, leakage between folds can be prevented. To simulate the test data, they downsampled training videos from fps=60 to fps=1. They also cropped the black empty space on the left and right side of all the training videos. Then, they blurred out the bottom banner which may contain ground truth labels. Finally, they resized the frames into 640 W x 512 H, the same as test videos.\\

After the above steps, the team trained ConvNext\cite{liu2022convnet} Tiny and EfficientNet\cite{tan2019efficientnet} B4 models, two model
architectures that consistently dominate Kaggle image competitions. Standard techniques were used such as cosine learning rate schedule, mixed precision training, mixup augmentations, and weighted loss functions. \\

Task 2 required localization and classification of a given set of surgical instruments in each frame of a video. Only video level labels were provided so the challenge can be tasked as a weakly supervised problem. In order to solve this problem they used a diversity of techniques taken from both supervised and unsupervised methods.\\

One of the key learnings from Task 1 was the importance of sampling rare classes and identifying high confidence labels in the train set. They exploited these learnings by developing a sample methodology to get a balanced set of frames/labels from a diverse set of scenes using the models they developed for Task 1. After these frames were identified they attempted to get clean localization of the tools of interest through two methods, GradCam\cite{selvaraju2017grad} and explicit labeling of the tools of interest. GradCam was effective at identifying the clevis of the tools of interest, however because there were a set of rules and detection logic that needed to be applied on top of the clevis identification (i.e., tip vs clevis detection for some tools and not others), they found that applying manual labels that incorporated these rules was important. GradCam was thus used for visualization only, and manual application of labels and competition logic were used for the start of training.

After identifying clean labels, the team trained YoloV5\cite{Jocher_YOLOv5_by_Ultralytics_2020} models first on a small set of manually created labels, according to the example labels on the challenge data page\footnote{https://surgtoolloc.grand-challenge.org/data/}, and then on weakly supervised pseudo-labels predicted from the first set of base models \cite{wang2021weakly}. The workflow is illustrated in Figure \ref{fig:nvtask2}.\\


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{TeamDocs/NVIDIA/task2.png}
    \caption{Team NVIDIA Task 2 workflow}
    \label{fig:nvtask2}
\end{figure}

\subsubsection{Model Training}
% \noindent training hyer-parameters, batch size, total epoch/iteration, random seed (if any).\\
% \noindent data preparation, pre-processing, etc.\\
% \noindent hardware settings for compute, CPU, GPU, etc.

For task 1, they trained 5 EfficientNet-B4 models (on 5 fold splits) and 5 ConvNext-tiny models, and ensembled them using a trick called logit shift. The idea of the logit shift trick is that, when data is extremely imbalanced between classes as in this dataset, the minor classes probabilities are extremely biased towards 0. The extent of the bias can be different across models, making ensembling difficult. Logit shifting is to shift the logit of each class by an optimal constant value (i.e. the same value for the same class, across all samples), so that 0.5 probability threshold is the optimal threshold for the F1 score. This optimal logit shift is tuned on local validation, and different for each model. When ensembling, they shift logit first on individual models then simply take the average probabilities, since they are already
adjusted to be centered around 0.5.\\

For task 2, the team trained several versions of YoloV5, and found YoloV5m to be the best performing. Except for the default augmentations such as mixup, mosaic and hsv transforms, they applied more augmentations like hue saturation value and random brightness contrast to make the model generalize better, especially for the minor tools.

All the experiments for the challenge was trained on NVIDIA DGX Station A100 (with A100 GPUs) and NVIDIA DGX Station (with V100 GPUs).

\subsubsection{Preliminary Performance}
% \noindent training, validation, testing performance\\
% \noindent (optional) table of performance results

For Task 1, The per-class F1 validation scores of both the ConvNext and EfficientNet models are provided in Table \ref{table:nv1}, as well as the ensemble score. The final ensemble has validation score 0.8526 and leaderboard score 0.7055.\\

For Task 2, the team achieved a mAP validation score of 0.3614 for the first model, and 0.4132 for the retrained model, which translated to leaderboard score 0.3058. The validation scores for each class is shown in Table \ref{table:nv2}.

\begin{table}[]
\begin{tabular}{lccc}
\hline
\centering
Class                          & ConvNext   Tiny & EfficientNet   B4 & Ensemble \\ \hline
needle driver                  & 0.9439          & 0.9565            & 0.9487   \\
cadiere forceps                & 0.6529          & 0.6826            & 0.6907   \\
bipolar forceps                & 0.9236          & 0.9305            & 0.9264   \\
monopolar curved scissors      & 0.9179          & 0.9330            & 0.9189   \\
grasping retractor             & 0.7082          & 0.6801            & 0.7188   \\
prograsp forceps               & 0.7549          & 0.7946            & 0.7742   \\
force bipolar                  & 0.9216          & 0.8665            & 0.9401   \\
vessel sealer                  & 0.9690          & 0.9728            & 0.9805   \\
permanent cautery hook/spatula & 0.8602          & 0.8417            & 0.8489   \\
clip applier                   & 0.8664          & 0.8700            & 0.8439   \\
tip-up fenestrated grasper     & 0.5333          & 0.5502            & 0.5222   \\
stapler                        & 0.9746          & 0.9748            & 0.9789   \\
bipolar dissector              & 0.9787          & 0.9744            & 0.9829   \\
suction irrigator              & 0.8619          & 0.8306            & 0.8619   \\ \hline
\textbf{Average   F1}                   & \textbf{0.8476}          & \textbf{0.8470}            & \textbf{0.8526}   \\ \hline
\end{tabular}
\caption{Team NVIDIA Task 1 Results}
\label{table:nv1}
\end{table}


\begin{table}[]
\begin{tabular}{lll}
\hline
\centering
Class                      & Frist model & Weakly supervised model \\ \hline
needle driver              & 0.5043      & 0.4933                  \\
cadiere forceps            & 0.5024      & 0.5111                  \\
bipolar forceps            & 0.3275      & 0.4441                  \\
monopolar curved scissors  & 0.3568      & 0.3898                  \\
grasping retractor         & 0.3101      & 0.4098                  \\
prograsp forceps           & 0.3619      & 0.4177                  \\
force bipolar              & 0.4341      & 0.4442                  \\
vessel sealer              & 0.4660      & 0.4874                  \\
permanent cautery hook     & 0.3866      & 0.4164                  \\
clip applier               & 0.2536      & 0.3520                  \\
tip-up fenestrated grasper & 0.4815      & 0.4472                  \\
stapler                    & 0.2262      & 0.2902                  \\
bipolar dissector          & 0.1046      & 0.3197                  \\
suction irrigator          & 0.3448      & 0.3617                  \\ \hline
\textbf{Average   mAP }             & \textbf{0.3614 }     & \textbf{0.4132}                  \\ \hline
\end{tabular}
\caption{Team NVIDIA Task 2 Results}
\label{table:nv2}
\end{table}

%\bibliographystyle{plain}
%\bibliography{nvidia}
%\end{document}


==> TeamDocs2022/SK/team_sk_orig.tex <==
%\documentclass{article}

%\usepackage{graphicx}

%\begin{document}

\subsection{Team SK} 

\begin{itemize}
  \item Team name: SK
  \item Members: Satoshi Kondo (Muroran Institute of Technology), Satoshi Kasai (Niigata University of Health and Welfare), Kousuke Hirasawa (Konica Minolta, Inc.)
  \item Categories:1, 2
  \item General motivation: Weakly-supervised surgical tool localization
\end{itemize}

\subsubsection{Method Description}

\paragraph{Overview}

They propose a weakly-supervised surgical tool localization method with multiplicative feature fusion network. Their network is trained to learn presence of surgical tools in the input image with supervised learning. When detecting surgical tools (task in category 1), they predict the presence of surgical tools by using the trained network. When localizing surgical tools (task in category 2), they once predict the presence of surgical tools, then they check the class activation map corresponding to the predicted surgical tool and localize the tool by thresholding the activation map, i.e., as weakly-supervised manner.


\paragraph{Details}

Figure 1 shows the entire structure of the proposed network. They use Multiplicative Feature Fusion Networks (MFF-Net) [1] as their base networks. MFF-Net is designed to aggregate features at different levels, which generates the class activation map (CAM) and categorical features for classification. They obtain CAM of the size $C \times H' \times W'$. Here, $C$ is the number of classes in the tool classification, and $H'$ and $W'$ are height and width of the CAM, respectively. They use ResNet-50 as the backbone in MFF-Net. The training and prediction are performed frame-by-frame base although the input data is video.

The network is trained by using the dataset, which has images and labels showing the presence of tools in the images. There are 14 surgical tools, and 3 tools are shown in an image at most. Based on their observation that two ``needle driver'' tools are often shown in the same images, they train their model not as 14-class classification model but 15-class classification model, i.e., $C=15$. They have two ``needle driver'' classes in 15 classes. When only one needle driver is shown in the input image, only the first label in needle driver classes is active, i.e., give 1 as the ground truth label. When two needle drivers are shown in the input image, both labels for needle driver classes are active.

In inference, the probabilities of surgical tool presence are obtained from the CAMs through global averaging pooling and sigmoid activation. They select the tool classes whose probabilities are higher than the threshold (0.5). The selected tool classes are the results for the surgical tool detection task (category 1). For the selected tools, they obtain CAM of the corresponding tool class in the order of the probability (from the highest probability to the lower ones). They obtain the tool area by thresholding the CAM. The threshold is decided by Otsu's binarization method. They identify the bounding box surrounding the tool area, and IoU is calculated when other bounding boxes are already allocated in the current image. If the IoU is less than the threshold, the bounding box is employed as the results of the surgical tool localization (category 2).

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{TeamDocs/SK/fig_sk.eps}
\caption{Overview of our proposed method.}
\label{fig:overview}
\end{figure}

\subsubsection{Model Training}

For the training of the network, they construct a dataset by sub-sampling images from videos. The total number of images for training is about 150k. They split the dataset to training and validation dataset in 8:2 ratio.

The augmentations are horizontal flip, shift, scale, rotation, color jitter, Gaussian blur and Gaussian noise. The augmented images are resized to $640 \times 480$ pixels. The optimizer is Adam, and the initial learning rate is $1.0 \times 10^{-5}$ changing at every epoch with cosine annealing. The loss function is cross-entropy loss. The batch size is 64 and the number of epochs is 30. The model taking the lowest loss value for the validation dataset is selected as the final model. They train five models by using 5-fold cross validation, and CAMs obtained by five models are averaged in inference. They use NVIDIA RTX3090 GPU for the training.

\subsubsection{Preliminary Performance}

They evaluated their method with the evaluation system provided by the challenge organizers. For category 1 (surgical tool detection), the F1 score was 0.816. For category 2 (surgical tool localization), mAP was 0.03.

%\subsubsection{References}

%[1] Wei, J., Wang, Q., Li, Z., Wang, S., Zhou, S. K., Cui, S. (2021). Shallow feature matters for weakly supervised object localization. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 5993-6001).

%\end{document}



==> TeamDocs2023/PUMCH/PUMCH.tex <==
\subsection{PUMCH}
\begin{itemize}
  \item Team name:  PUMCH
  \item Members:  Surong Hua, Lu Ping, Wenming Wu
  \item Research field: Computer Vision
  \item Institution: Peking Union Medical College Hospital
  \item City: Beijing, China
  \item motivation and plan: At first glance, we were thinking of weakly supervised learning. But then we found that the video tags provided for training only contain information on whether a certain instrument exists in this video, it was not certain that whether the instrument appears in every frame, since it might be partially or completely obscured, which reduced the performance. 
  We also noticed that almost all the winning teams last year were based on semi-supervised method. Therefore, we proposed a framework by combining semi-supervised learning, object detection, and object tracking together.
\end{itemize}
 
\subsubsection{Method Description}

\paragraph{Data Processing}
See Figure \ref{fig:fig1} ,in this framework, we adopt the following three methods to process data. Firstly, for frames without labels, We use the MAE\cite{He_Chen_Xie_Li_Dollar_Girshick_2022} method to train the feature extraction ability of the backbone network. Secondly, we referred to last year's champion method to merge and process consecutive video segments to get sequence information, and then manually annotate the target in multiple stages of the video. Then, we used a transformer-based target tracking model (ostrack)\cite{Ye_Chang_Ma_Shan} to generate pseudo labels. Thirdly, we use tools presence labels to conduct cross validation and manual correction. Then, the model is continuously looped and trained to update pseudo labels. Ultimately, we obtained 30,000 pseudo label data.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{TeamDocs2023/PUMCH/fig1.png}
    \caption{Data Processing}
    \label{fig:fig1}
\end{figure}

\paragraph{Architecture Design}
Specifically, As Figure \ref{fig:fig2} shows, OStrack\cite{Ye_Chang_Ma_Shan} in our strategy consists of the following four steps: (1) The template and search region undergo patch embedding and spreading to recover the token, which is added with the positional encoding and spliced to form the overall token. (2) The overall token is fed into the encoder, in which the similarity between each token and the template token is calculated, and the foreground token is retained while the background token is rounded off in descending order. 
(3) Token padding is then performed to complement the rounded tokens with zeros and output to the head. (4) The head section outputs the classification score, the predicted offset value to compensate for down-sampling quantization error, and the normalized bounding box size, respectively.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{TeamDocs2023/PUMCH/fig2.png}
    \caption{OsTrack Pipeline}
    \label{fig:fig2}
\end{figure}
\paragraph{Model Loss Function}
To train the one-stage object detector,we adpoted a dynamic soft label assignment strategy based on SimOTA \cite{Ge_Liu_Wang_Li_Sun_Technology}.As RTM-DET \cite{Lyu_Zhang_Huang_Zhou_Wang_Liu_Zhang_Chen_Conv_Concat}does,we used the IoU between the predictions and ground truth boxes as the soft label to train the classification branch,used the logarithm of the IoU as the regression cost instead of GIoU used in the loss function, used a soft center region cost instead of a fixed center prior  to stabilize the matching of the dynamic cost.

\paragraph{Post Processing}
We adopted Kalman filtering approach based on weighted boxes fusion (WBF) \cite{Solovyev_Wang_Gabruseva_2021} to achieve a higher detection rate.To be specific, the implementation of WBF has the following steps: (1) The prediction frames of both the detection and the tracking model are normalized by coordinates and confidence, and clustered into a single set B and sorted in descending order using the confidence of the detection frames. (2) two empty lists are initialized, list one is used to hold clusters of detection frames for each target and list two is used to hold fusion frames for each target. (3) The algorithm would iterate through the predictions in B and calculate Intersection over Union (IoU) with each fused frame in list two. (3) When IOU is greater than a manually set threshold “T”, the clusters are considered to be in the same class, and coordinates and confidence of the fused frames are calculated. On the other hand, when IOU is smaller than T, the new box is defined as a new cluster center and is added to the tails of list one and list two. Then the iterative traversal for all the boxes in B is repeated. Eventually the box in List two would be the result.

\subsubsection{Model Training}
\paragraph{Long Tail}
As We noticed that our test metric is MAP, and we realized that the 14 low frequency instruments have long tail distributions, which will lead to the model overfitting,see Figure \ref{fig:fig3} .To avoid this, we utilized the tools presence labels to generate pseudo labels in similar size by instrument categories.

\paragraph{Implementation Details}
We divided all the data into a training set and a validation set by 7:3, and then conducted model experiments, data augmentation, category balance, and ensemble experiments, respectively. For every experiment, we trained our models on the training set for 100 epochs and validated them on the validation set. The hyper-parameters are in Table 1. All experiment  were trained on 8 NVIDIA A100 GPUs. We evaluate the model performance on object detection and instance segmentation by bbox AP.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{TeamDocs2023/PUMCH/fig3.png}
    \caption{Long Tail}
    \label{fig:fig3}
\end{figure}

\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Config}        & \textbf{Training Setting} \\ \hline
Optimizer              & AdamW                     \\ \hline
Optimizer Monentum     & 0.9                       \\ \hline
Learning Rate          & 0.004                     \\ \hline
Learning Rate Schedule & Flat-Cosine               \\ \hline
Weight Decay           & 0.05                      \\ \hline
Training Epochs        & 100                       \\ \hline
Warmup Iterations      & 1000                      \\ \hline
Input Size             & 640x640                   \\ \hline
Batch Size             & 64                        \\ \hline
\end{tabular}
\caption{ Training Settings}
\label{table:table0}
\end{table}




\subsubsection{Preliminary Performance}
\paragraph{Results}
Tab2-Tab6  show which modules perform best on the current validation set.Then, we choose RTM-DET \cite{Lyu_Zhang_Huang_Zhou_Wang_Liu_Zhang_Chen_Conv_Concat} as our detection model, cbnet-swim \cite{Liu_Wang_Wang_Liang_Zhao_Tang_Ling_2020} as our backbone, auto-augment as data augmentation, and adopt category balancing strategy. Finally, we adopted the integration of RTM-DET and the fine-tuned tracking model as our final submission.

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Model}          & \textbf{Size} & \textbf{Bbox\_map} \\ \hline
Cascade R-CNN-Detectors & (894,682)     & 63.6               \\ \hline
RTMDet-l                & (864,864)     & 70.6               \\ \hline
YOLOv8-l                & (864,864)     & 69.1               \\ \hline
Co-DETR-swin-s          & Multi   scale & 64.6               \\ \hline
\end{tabular}
\caption{ Model Experiments}
\label{table:table1}
\end{table}



\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Backbone}    & \textbf{Bbox\_map} \\ \hline
cspnext              & 70.6               \\ \hline
Convnext             & 70.6               \\ \hline
Convnext-v2          & 70.9               \\ \hline
swintransformer\_7   & 70.6               \\ \hline
swintransformer\_12  & 71.1               \\ \hline
Swintransformer\_MAE & 66.0               \\ \hline
resnet               & 63.6               \\ \hline
convnext             & 70                 \\ \hline
Cbnet\_swin          & 71.5               \\ \hline
Cbnet\_res2net101    & 70.1               \\ \hline
\end{tabular}
\caption{ Backbone Experiments}
\label{table:table2}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Data Augmentation}                             & \textbf{Bbox\_map} \\ \hline
Mosaic\_mixup                                          & 70.6               \\ \hline
Mosaic\_mixup9                                         & 70.8               \\ \hline
Fog-Blur-Noise and   channelshiift                     & 71.2               \\ \hline
RandomBrightnessContrast   MotionBlur ShiftScaleRotate & 71.1               \\ \hline
Autoaugment                                            & 71.2               \\ \hline
convnext                                               & 70                 \\ \hline
Cbnet\_swin                                            & 71.5               \\ \hline
Cbnet\_res2net101                                      & 70.1               \\ \hline
\end{tabular}
\caption{ Data Augmentation Experiments}
\label{table:table3}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Class Balance} & \textbf{Bbox\_map} \\ \hline
w/o                    & 70.6               \\ \hline
w                      & 71.4               \\ \hline
\end{tabular}
\caption{ Class Balance experiments}
\label{table:table4}
\end{table}


\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
Model              & Fusion    & \textbf{Bbox\_map} \\ \hline
rtmdet-siamfcpp    & wbf\_mean & 65                 \\ \hline
rtmdet-OStrack     & wbf\_mean & 66.7               \\ \hline
rtmdet-OStrack\_FT & wbf\_mean & 67.9               \\ \hline
rtmdet-OStrack\_FT & wbf\_max  & 64.2               \\ \hline
\end{tabular}
\caption{ Ensemble experiments}
\label{table:table5}
\end{table}


\paragraph{Conclusion and Discussion}
We have adopted the method of integrating detection models with tracking models. Although it has shown effectiveness in offline evaluations, it has not shown greater advantages in online evaluations. We believe that the online test set may be more complex, and our tracking model does not perform well. Compared to the previous semi supervised schemes, we have introduced self supervised learning, optimized the detection and tracking models, and considered class imbalance, which are still directions for future optimization.

